Towards Accurate and Efficient Document Analytics with Large Language Models

Unstructured data formats account for over 80% of the data currently stored, and extracting value from such formats remains a considerable challenge. In particular, current approaches for managing unstructured documents do not support ad-hoc analytical queries on document collections. Moreover, Large Language Models (LLMs) directly applied to the documents themselves, or on portions of documents through a process of Retrieval-Augmented Generation (RAG), fail to provide high accuracy query results, and in the LLM-only case, additionally incur high costs. Since many unstructured documents in a collection often follow similar templates that impart a common semantic structure, we introduce ZenDB, a document analytics system that leverages this semantic structure, coupled with LLMs, to answer ad-hoc SQL queries on document collections. ZenDB efficiently extracts semantic hierarchical structures from such templatized documents, and introduces a novel query engine that leverages these structures for accurate and cost-effective query execution. Users can impose a schema on their documents, and query it, all via SQL. Extensive experiments on three real-world document collections demonstrate ZenDB's benefits, achieving up to 30% cost savings compared to LLM-based baselines, while maintaining or improving accuracy, and surpassing RAG-based baselines by up to 61% in precision and 80% in recall, at a marginally higher cost.

==> usecase.tex <==
\section{Use Case Scenarios}
\label{sec:usecase}

% \yiming{We plan to use civic council notes, systematic review, and historical study as three use cases. Briefly describe each use case with sample data and queries to demonstrate 1) the complexity of the text as mentioned in the introduction; 2) and make sense of query workloads on each data set; 3) the need of TEXT-DB to support advanced analytics on text. }
We collected several real-world use case scenarios from diverse areas in civic agenda reporting, historical study and systematic review by interviewing users or researchers from their projects. 

\noindent\textbf{Civic Agenda.}
A large digital collections of civic agenda and minute meeting notes are being produced from local public meetings every day, which are important sources for decision maker to collect public comment, for the journalists to investigate news stories and for the public to understand the discussed items and their outcomes. Civic data can have diverse formats, heterogeneous structures and complex and large content. (e.g., Figure~\ref{fig:civic} shows one such example.) 
It is crucial for users to first make sense of such large scale and complex civic documents before they could issue any query. The queries, based on the interviewed reports from the journalists, could range from simple fact extraction (e.g., ``what is the discussed topic?'') to advanced queries such as aggregation (e.g., ``Does the majority of people vote yes or no for certain discussed topic in the meeting at Malibu City on March 27, 2023?''). People often do not fully believe the results produced by a learned machine learning model, and thus the provenance (i.e., the context where a query answer is generated from) maintenance is important for human verification.  Our system could be a good fit to help different users to utilize the civic documents by understanding the text, supporting advanced queries and providing provenance as well as accuracy estimation to gain the confidence of the result. 


\noindent\textbf{Historical Study.} 
We conducted interviews with historical researchers
from the First Historical Archives of China, an institution housing over four million digital historical records. Their goal is to develop a  tool that enables the public to engage in more detailed and insightful text-based analysis, enhancing their understanding of history. Additionally, this tool aims to aid historians in verifying and investigating historical facts more effectively. The historical data observed often possess varied structures, and the queries posed can be quite ad-hoc. A key vision of TEXT-DB is to facilitate advanced query analytics, improving the extraction of valuable insights from such unstructured textual data with better accuracy, lower latency and expense to finally support a possibly interactive analytics. This enhancement is intended to assist both the general public and researchers in gaining a deeper comprehension of historical events.

%We interviewed the historical researchers from the first historical archives of China, where over 4 millions digital historical archives are stored. They tried to create a better tool to help the public to explore richer and fine-grained analytics on text to know the history better, and also support historical researchers to verify and explore historical facts for a more efficient research purpose. The observed historical data are typically with diverse structure and the queries could be extremely ad-hoc. One of TEXT-DB's vision is to support the advanced query analytics to better extract values from such unstructured text data in the wild to help the public and researchers to better know the histories. 

\noindent\textbf{Systematic Review.} 
Researchers often conduct systematic review to make sense of a particular research topic or questions by reviewing existing research publications. They typically take a set of related publications as input by using keyword or embeddings search over the internet. Then they conduct various detailed queries like ``what are the domain/theory/motivation of the publications from which conference in what time range?''. This process is typically iterative since researchers need to refine the taxonomies based on the retrieved content where the provenance is useful. Then they may conduct aggregate/group by queries where each taxonomy is a group to visualize the query results. TEXT-DB can help speed up such an iterative exploration by providing accurate provenance for human refinement as well as fast approximation of visualizations without looking at each entire paper line by line, which can be extremely labor-intensive. 
